Pearls from Pebbles: Improved Confidence Functions for Auto-labeling

Auto-labeling is an important family of techniques that produce labeled training sets with minimum manual labeling. A prominent variant, threshold-based auto-labeling (TBAL), works by finding a threshold on a model's confidence scores above which it can accurately label unlabeled data points. However, many models are known to produce overconfident scores, leading to poor TBAL performance. While a natural idea is to apply off-the-shelf calibration methods to alleviate the overconfidence issue, such methods still fall short. Rather than experimenting with ad-hoc choices of confidence functions, we propose a framework for studying the \emph{optimal} TBAL confidence function. We develop a tractable version of the framework to obtain \texttt{Colander} (Confidence functions for Efficient and Reliable Auto-labeling), a new post-hoc method specifically designed to maximize performance in TBAL systems. We perform an extensive empirical evaluation of our method \texttt{Colander} and compare it against methods designed for calibration. \texttt{Colander} achieves up to 60\% improvements on coverage over the baselines while maintaining auto-labeling error below $5\%$ and using the same amount of labeled data as the baselines.

==> sections/auto-lbl-opt-algo.tex <==
 
\begin{algorithm}[h]
\caption{Auto-labeling Optimization}
  \begin{algorithmic}[1]
  \Require $ \cG, \hat{\fh}_i,\Dcal$
  \Ensure  New confidence function $\hat{g}_i'$ 
  %\State $D_v = randomly\_query\_batch(\mathcal{X},n_v)$
 % \If {$|D_v^{(i)}|< n_v^{(i)}$}
 %     \State $z_i = n_v^{(i)}-|D_v^{(i)}| $
 %     \State $Z^{(i)} = \texttt{random\_query\_batch}(X_u^{(i)}, z_i) $
 %      \State $D_v^{(i)} = D_v^{(i)} \cup Z^{(i)}$
 %      \State Remove points in $D_v^{(i)}$ from $X_u^{(i)}$
  %\EndIf
    \State $$\hat{g}_i,\hat{u}_i =  \argmin_{g \in \cG, t \in T} \quad  -\surrcov(g,t \given h) 
+ \lambda\, \surrerr(g,t \given h) $$
  \end{algorithmic}
  %\land  |\hat{R}_{t}(\hat{h}_i,X_v^{(i)}) - R_{t}(h_i,\mathcal{X}_u^{(i)}) | \le \epsilon/2
  
  \label{alg:gamma-estimate}

\end{algorithm}





==> sections/fig-tex/fig-bar-main-table.tex <==

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/error_and_coverage.png}
    \caption{(a)-(d) illusrate the auto-labeling error for ours and the baseline methods on MNIST, CIFAR-10, 20 Newsgroup, and Tiny-Imagenet respectively; (e)-(h) illusrate the covreage for ours and the baseline methods on MNIST, CIFAR-10, 20 Newsgroup, and Tiny-Imagenet respectively.}
    \label{fig:error_and_coverage}
\end{figure*}

==> sections/fig-tex/g_figure.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/TBAL_al_optimizationv0_2.png}
    \vspace{-5pt}
    \caption{Illustration of our choice of $\fg$ functions. The concatenation of the last two layers representations from the classification model $\fh$ is used as the input for confidence function $\fg$.}
    \label{fig:illu_our}
    \vspace{-15pt}
\end{figure}


==> sections/fig-tex/solution_space_fig.tex <==

\begin{figure}[t]
%\vspace{-13pt}
\centering
{\includegraphics[width=\linewidth]{figs/sol_space.pdf}}
\vspace{-20pt}
\caption[]{ \small{Illustration of solution space of problem \eqref{eq:true_opt}. We use a toy data setting of $x \sim \mathrm{Unif}(0,1)$ with $1-$d threshold classifier $\fh_{\theta}(x) = \one(x\ge \theta)$. For any $x$, let true labels $y=\fh_{0.5}(x)$ and consider the confidence function $\fg_w(x)=(w-x)^2$. Let $\hat{y} = \fh_{0.25}(x)$ and consider the points on the side where $\hat{y}=1$. }}
\label{fig:sol_space}
\vspace{-10pt}
\end{figure}

==> sections/fig-tex/surrogate_good_backup.tex <==

%{\color{red} write about active querying strategy, it is same as in previous paper. we use softmax scores for this, to avoid confounding/conflating. It is an interesting question to see if using our g in active querying could further improve the performance. }

\begin{figure}[h]
  \begin{minipage}{0.5\linewidth}
    \subfigure[ Contours of Surrogate and Actual Functions\label{fig:contours}]{\includegraphics[width=\textwidth]{figs/contours.pdf}}
  \end{minipage}
  \hfill
  \begin{minipage}{0.5\linewidth}
    \mbox{
    \subfigure[ Auto-labeling error and surrogate error at various $\alpha$.\label{fig:surr_err}]{\includegraphics[width=\textwidth]{figs/surrogate_err_all_alpha.pdf}}
  }
    \mbox{
    \subfigure[ Auto-labeling coverage and surrogate coverage at various $\alpha$.\label{fig:surr_cov}]{\includegraphics[width=\textwidth]{figs/surrogate_cov_all_alpha.pdf}}
  }
  \end{minipage}
  \caption{Illustration of the tightness of surrogate error and coverage functions based on the choice of $\alpha$. We use a toy data setting of $x \sim \mathrm{Uniform}(0,1)$ with $1-$dimensional threshold classifier $\fh_{\theta}(x) = \one(x\ge \theta)$. For any $x$, let true labels $y=\fh_{0.5}(x)$ and consider the confidence function $\fg_w(x)=|w-x|$. Let $\hat{y} = \fh_{0.25}(x)$ and consider the points on the side where $\hat{y}=1$. We plot the actual and surrogate errors in (b), and the surrogate and actual coverage in (c).}
  \label{fig:example-key}
\end{figure}

==> sections/impact.tex <==
\section{Impact Statement}
This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.



==> tables/v0/passive_cifar10_med_net.tex <==


\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 2.709 $\pm$ 0.547              & 11.060 $\pm$ 1.462             \\
        Ours                           & Vanilla                        & 2.028 $\pm$ 0.285              & \textbf{49.628 $\pm$ 0.692}    \\
        Dirichlet                      & Vanilla                        & 2.981 $\pm$ 0.321              & 11.227 $\pm$ 2.102             \\
        Histogram binning top label    & Vanilla                        & \textbf{1.837 $\pm$ 0.620}     & 5.506 $\pm$ 1.087              \\
        Scaling binning                & Vanilla                        & 2.727 $\pm$ 0.348              & 9.759 $\pm$ 1.334              \\
        Temperature scaling            & Vanilla                        & 3.047 $\pm$ 0.495              & 12.037 $\pm$ 1.981             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for training-time methods via passive learning on cifar10 med net calib 0 passive learning eval full/cifar10 med net dataset.}
    \label{table:cifar10_med_net_calib_0_passive_learning_eval_full/cifar10_med_net_passive_learning__01-15-2024__12-16-39}
\end{table*}


==> tables/v0/passive_cifar10_resnet18.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 2.471 $\pm$ 0.166              & 18.708 $\pm$ 0.561             \\
        Ours                           & Vanilla                        & \textbf{1.903 $\pm$ 0.220}     & \textbf{53.837 $\pm$ 0.333}    \\
        Dirichlet                      & Vanilla                        & 2.776 $\pm$ 0.213              & 20.812 $\pm$ 1.047             \\
        Histogram binning top label    & Vanilla                        & 2.044 $\pm$ 0.262              & 12.959 $\pm$ 2.103             \\
        Scaling binning                & Vanilla                        & 2.467 $\pm$ 0.052              & 17.572 $\pm$ 2.235             \\
        Temperature scaling            & Vanilla                        & 2.928 $\pm$ 0.075              & 19.358 $\pm$ 1.640             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for training-time methods via passive learning on pl cifar10 resnet18 dataset.}
    \label{table:pl_cifar10_resnet18_passive_learning__01-17-2024__00-24-15}
\end{table*}

==> tables/v0/passive_cifar10_small_net.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 5.026 $\pm$ 0.482              & 2.142 $\pm$ 0.495              \\
        Ours                           & Vanilla                        & \textbf{1.915 $\pm$ 0.341}     & \textbf{39.494 $\pm$ 0.625}    \\
        Dirichlet                      & Vanilla                        & 6.850 $\pm$ 1.824              & 3.165 $\pm$ 0.117              \\
        Histogram binning top label    & Vanilla                        & 6.762 $\pm$ 1.403              & 1.493 $\pm$ 0.458              \\
        Scaling binning                & Vanilla                        & 11.205 $\pm$ 2.378             & 0.978 $\pm$ 0.697              \\
        Temperature scaling            & Vanilla                        & 6.916 $\pm$ 1.252              & 3.377 $\pm$ 0.618              \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for training-time methods via passive learning on cifar10 small net calib 0 passive learning eval hyp/cifar10 small net dataset.}
    \label{table:cifar10_small_net_calib_0_passive_learning_eval_hyp/cifar10_small_net_passive_learning__01-15-2024__21-10-55}
\end{table*}

==> tables/v0/passive_mnist.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & \textbf{2.111 $\pm$ 0.379}     & 77.692 $\pm$ 2.786             \\
        Ours                           & Vanilla                        & 3.777 $\pm$ 0.597              & \textbf{94.638 $\pm$ 1.266}    \\
        Dirichlet                      & Vanilla                        & 3.632 $\pm$ 0.689              & 81.704 $\pm$ 0.081             \\
        Histogram binning top label    & Vanilla                        & 3.745 $\pm$ 0.886              & 84.616 $\pm$ 5.500             \\
        Scaling binning                & Vanilla                        & 3.569 $\pm$ 0.791              & 83.512 $\pm$ 5.671             \\
        Temperature scaling            & Vanilla                        & 3.789 $\pm$ 0.885              & 84.548 $\pm$ 5.743             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for training-time methods via passive learning on mnist  dataset.}
    \label{table:mnist_lenet_passive_learning__01-15-2024__16-38-47}
\end{table*}

==> tables/v0/passive_tiny_imagenet.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 6.505 $\pm$ 0.417              & 20.521 $\pm$ 1.279             \\
        Ours                           & Vanilla                        & \textbf{2.154 $\pm$ 3.127}     & \textbf{38.189 $\pm$ 2.369}    \\
        Dirichlet                      & Vanilla                        & 12.275 $\pm$ 1.279             & 11.903 $\pm$ 0.695             \\
        Histogram binning top label    & Vanilla                        & 10.659 $\pm$ 0.622             & 13.634 $\pm$ 0.437             \\
        Scaling binning                & Vanilla                        & 10.326 $\pm$ 0.209             & 12.879 $\pm$ 1.126             \\
        Temperature scaling            & Vanilla                        & 10.902 $\pm$ 0.105             & 14.085 $\pm$ 1.133             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for vanilla training-time methods via passive learning on tiny imagenet CLIP dataset.}
    \label{table:tiny_imagenet_CLIP_passive_learning_vanilla}
\end{table*}

==> tables/v0/passive_twenty_newsgroup.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 3.869 $\pm$ 0.745              & 34.828 $\pm$ 3.408             \\
        Ours                           & Vanilla                        & \textbf{3.349 $\pm$ 1.162}     & \textbf{63.761 $\pm$ 0.894}    \\
        Dirichlet                      & Vanilla                        & 4.530 $\pm$ 1.405              & 36.975 $\pm$ 3.982             \\
        Histogram binning top label    & Vanilla                        & 4.665 $\pm$ 1.418              & 35.270 $\pm$ 7.548             \\
        Scaling binning                & Vanilla                        & 4.420 $\pm$ 1.163              & 36.176 $\pm$ 4.320             \\
        Temperature scaling            & Vanilla                        & 4.789 $\pm$ 0.969              & 38.592 $\pm$ 4.170             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for vanilla training-time methods via passive learning on twenty newsgroups dataset.}
    \label{table:twenty_newsgroups_passive_learning_vanilla}
\end{table*}


==> tables/v0/tbal_cifar10_med_net.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 6.965 $\pm$ 0.454              & 12.053 $\pm$ 1.040             \\
        Ours                           & Vanilla                        & \textbf{2.788 $\pm$ 0.241}     & \textbf{82.587 $\pm$ 0.192}    \\
        Dirichlet                      & Vanilla                        & 9.441 $\pm$ 0.521              & 12.559 $\pm$ 0.810             \\
        Histogram binning top label    & Vanilla                        & 6.153 $\pm$ 0.705              & 6.821 $\pm$ 2.183              \\
        Scaling binning                & Vanilla                        & 9.311 $\pm$ 3.525              & 4.372 $\pm$ 1.582              \\
        Temperature scaling            & Vanilla                        & 9.546 $\pm$ 0.488              & 15.984 $\pm$ 2.501             \\
        \bottomrule
    \end{tabular}
    \caption{TBAL( Multi-Round), CIFAR-10 + MediumNet.}
    \label{table:cifar10_med_net_calib_0_tbal_eval_full/cifar10_med_net_tbal__01-16-2024__13-16-22}
\end{table*}

==> tables/v0/tbal_mnist.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Post-hoc Method                & Training-time Method           & Auto-labeling Error            & Coverage                       \\
        \midrule
         -                             & Vanilla                        & 5.913 $\pm$ 1.845              & 84.236 $\pm$ 1.648             \\
        Ours                           & Vanilla                        & \textbf{3.780 $\pm$ 0.848}     & \textbf{95.329 $\pm$ 1.648}    \\
        Dirichlet                      & Vanilla                        & 9.181 $\pm$ 1.244              & 93.020 $\pm$ 0.685             \\
        Histogram binning top label    & Vanilla                        & 8.242 $\pm$ 1.386              & 92.487 $\pm$ 5.216             \\
        Scaling binning                & Vanilla                        & 7.515 $\pm$ 0.999              & 92.668 $\pm$ 1.953             \\
        Scaling binning                & Vanilla                        & 7.123 $\pm$ 1.149              & 92.866 $\pm$ 0.732             \\
        Temperature scaling            & Vanilla                        & 8.957 $\pm$ 0.692              & 94.324 $\pm$ 1.614             \\
        \bottomrule
    \end{tabular}
    \caption{Auto-labeling error and coverage of post-hoc methods for training-time methods via tbal on tbal mnist lenet dataset.}
    \label{table:tbal_mnist_lenet_tbal__01-16-2024__06-09-16}
\end{table*}
